EarthNet2021: A large-scale dataset and challenge for Earth surface forecasting as a guided video prediction task

Satellite images are snapshots of the Earth surface. We propose to forecast them. We frame Earth surface forecasting as the task of predicting satellite imagery conditioned on future weather. EarthNet2021 is a large dataset suitable for training deep neural networks on the task. It contains Sentinel 2 satellite imagery at 20m resolution, matching topography and mesoscale (1.28km) meteorological variables packaged into 32000 samples. Additionally we frame EarthNet2021 as a challenge allowing for model intercomparison. Resulting forecasts will greatly improve (>x50) over the spatial resolution found in numerical models. This allows localized impacts from extreme weather to be predicted, thus supporting downstream applications such as crop yield prediction, forest health assessments or biodiversity monitoring. Find data, code, and how to participate at www.earthnet.tech

==> sections/OLD02relatedwork.tex <==
\section{Related work}

\paragraph{Traditional approaches to the forecasting of Earth surface}
Our work relates to both spatial downscaling of climate or coarse-scale remote sensing data and to temporal forecasts. Temporal forecasts of vegetation state have been performed on km to 50 km scale \citet{tadesse2010,asoka2015,kraft2019}.  Approaches to downscale Earth surface conditions to <100m exist as well, but are not connected to temporal forecasts to our knowledge, but rather blending multiple observations \citet{ke2016}. 

\paragraph{ML approaches to the forecasting of Earth surface}
Using temporal context (\citet{kraft2019} and \citet{foley2020}) using spatial context (Chris). Both useful at improving performance, but no dataset available allow to use both spatial and temporal context -> Ideal for video prediction models.


==> sections/ideas2022.tex <==
EarthNet2022
    Go Worldwide
    Go to 10m/pix from 20m?pix
    Go 256x256
    Go with more sentinel bands
    Go with other source for weather (global)
    Add GLiM predictor (soil/geology)
    Add QQ
    Improve metrics based on learnings from 2021
    DL based cloud mask
    
    Evaluate ensemble using rank statistics see: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9246532
